Continual Learning in Neural Networks

Artificial neural networks have exceeded human-level performance in accomplishing several individual tasks (e.g. voice recognition, object recognition, and video games). However, such success remains modest compared to human intelligence that can learn and perform an unlimited number of tasks. Humans' ability of learning and accumulating knowledge over their lifetime is an essential aspect of their intelligence. Continual machine learning aims at a higher level of machine intelligence through providing the artificial agents with the ability to learn online from a non-stationary and never-ending stream of data. A key component of such a never-ending learning process is to overcome the catastrophic forgetting of previously seen data, a problem that neural networks are well known to suffer from. The work described in this thesis has been dedicated to the investigation of continual learning and solutions to mitigate the forgetting phenomena in neural networks. To approach the continual learning problem, we first assume a task incremental setting where tasks are received one at a time and data from previous tasks are not stored. Since the task incremental setting can't be assumed in all continual learning scenarios, we also study the more general online continual setting. We consider an infinite stream of data drawn from a non-stationary distribution with a supervisory or self-supervisory training signal. The proposed methods in this thesis have tackled important aspects of continual learning. They were evaluated on different benchmarks and over various learning sequences. Advances in the state of the art of continual learning have been shown and challenges for bringing continual learning into application were critically identified.

==> chapters/abbreviations/abbreviations.tex <==
% !TeX root = ../../thesis.tex
\chapter{List of Abbreviations}    
\label{ch:abbreviations}
\vspace{-10pt}
\begin{tabular}{ll}
%CL & \tab Continual Learning\\\\
EBLL &\tab Encoder Based Lifelong Learning \\\\
EG &\tab Expert Gate \\\\
EWC& \tab Elastic Weight Consolidation \\\\
LwF  & \tab Learning without Forgetting \\\\
GEM &\tab Gradient Episodic Memory \\ \\
iCaRL &\tab Incremental Classifier and Representation Learning \\ \\
i.i.d. &\tab  Independent and identically distributed\\ \\
 IMM &\tab Incremental Moment Matching \\ \\
 MAP &\tab    Maximum A posteriori Probability  estimate\\ \\
 MAS &\tab Memory Aware Synapses \\\\
 MLE &\tab  Maximum Likelihood Estimation\\ \\
 PCA &\tab    Principal Component Analysis\\ \\
  SCL &\tab Selfless Continual Learning \\ \\
 SI &\tab Synaptic Intelligence \\\\
 SVD &\tab     Singular Value Decomposition\\ \\

\end{tabular}


% \begin{tabular}{ll}
% %CL & \tab Continual Learning\\\\
% LwF  & \tab Learning without Forgetting \\\\
% EG &\tab Expert Gate \\\\
% EBLL &\tab Encoder Based Lifelong Learning \\\\
% EWC& \tab Elastic Weight Consolidation \\\\
%  MAS &\tab Memory Aware Synapses \\\\
%  SI &\tab Synaptic Intelligence \\\\
%  IMM &\tab Incremental Moment Matching \\ \\
%   SCL &\tab Selfless Continual Learning \\ \\
%     iCaRL &\tab Incremental Classifier and Representation Learning \\ \\
%     GEM &\tab Gradient Episodic Memory \\ \\
% i.i.d. &\tab  Independent and identically distributed\\ \\
% MLE &\tab  Maximum Likelihood Estimation\\ \\
% MAP &\tab    maximum a posteriori probability  estimate\\ \\
% PCA &\tab    Principal Component Analysis\\ \\
%  SVD &\tab     Singular value decompositions\\ \\

% \end{tabular}


% CL\, \, \, \tab Continual Learning \\\\
% LwF \,\tab Learning without Forgetting \\\\
% EG\, \, \, \tab Expert Gate \\ \\
% EBLL \tab Encoder Based Lifelong Learning \\ \\
% EWC\, \tab Elastic Weight Consolidation \\ \\
% MAS\, \tab Memory Aware Synapses \\ \\
% SI\, \, \, \, \tab Synaptic Intelligence \\ \\
% IMM \,\tab Incremental Moment Matching \\ \\

\cleardoublepage

==> chapters/abstract/abstract.tex <==
% !TeX root = ../../thesis.tex
\chapter{Abstract}                                 \label{ch:abstract}

%\ldots

%\instructionsabstract

Artificial neural networks have exceeded human level performance in accomplishing several individual tasks (e.g. voice recognition, object recognition, and video games). However, such success remains modest compared to  human intelligence that can learn and perform an unlimited number of tasks. Humans ability of learning and accumulating knowledge over their lifetime is an essential aspect of their  intelligence.
In this respect, continual machine learning aims at a higher level of machine intelligence through providing the artificial agents with the ability to learn online from a non-stationary and never-ending stream of data. 

A key component of  such a never-ending learning process is to overcome the catastrophic forgetting of previously seen data, a problem that neural networks are well known to suffer from.
The work described in this thesis has been dedicated to the investigation of  continual learning  and solutions to mitigate the forgetting phenomena in neural networks.

To approach the continual learning problem, we first assume a task incremental   setting where tasks are received one at a time and data from previous tasks are not stored.  
We start by developing a system that aims for  an expert level performance on each learned task. It  reserves  a separate specialist model for each task and sequentially learns a gate to forward the input data to the corresponding specialist. We then  consider the incremental learning of multiple tasks using a  shared model of fixed capacity.  For each task, we identify  the most informative  features and minimize their divergence during the learning of later tasks; using as a proxy the current task data.

As an alternative to relying on the current task data, which might be of a very different distribution than previous data, important parameters in a model can be identified and future changes  on them get penalized. However, when accounting for an unlimited sequence of tasks, it is impossible to preserve all the previous knowledge. As an adaptive method to specific test conditions, we propose to learn the important parameters at deployment time  while the model is active in its test environment. As a result, catastrophic forgetting is overcome but graceful selective forgetting is tolerated. 
To further account for future tasks, we study the role of sparsity in continual learning. We propose a new regularizer that significantly reduces the percentage of parameters dedicated to each task and as a consequence remarkably improves the continual learning performance. 

Since the task incremental   setting can't be assumed in all continual learning scenarios,  we also study the more general online continual setting. We consider an infinite stream of data drawn from a non-stationary distribution with a supervisory or self-supervisory training signal.  We first propose a protocol to bring our work on regularizing the important parameters to the online continual learning setting and show an improved learning performance over different streams of data.  As to account for more challenging situations where the input distribution is experiencing bigger changes, we explore the use of a fixed buffer of samples selected from the previous history.  We propose a sample selection method that makes no assumption on the data generating  distribution.  To the best of our knowledge, we were the first to tackle the online continual learning problem. 

The proposed methods  in this thesis  have tackled  important aspects of continual learning. They were evaluated on different benchmarks and over various learning sequences. Advances in the state of the art of continual learning have been shown and challenges for bringing continual learning into application were critically identified.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/abstractnl/abstractnl.tex <==
% !TeX root = ../../thesis.tex
\chapter{Beknopte samenvatting}
    \label{ch:abstractnl}
Artificiële neurale netwerken scoren voor vele individuele taken (bv. Spraakherkenning, objectherkenning en videospellen) beter dan de mens. Het succes blijft echter beperkt, als we kijken naar  het oneindig aantal taken dat een mens kan leren en uitvoeren. De mogelijkheid om een leven lang te leren en kennis te blijven vergaren, is een essentiël typering van menselijke intelligentie. Met dit in gedachte mikt continu leren op een hoger niveau van machinale intelligentie, door de artificiële intelligentie de mogelijkheid te bieden om on-line te blijven leren met een oneindige stroom aan data. Een cruciale component in zo’n nooit eindigend leerproces is het overwinnen van het rampzalige vergeten van eerder verkregen data, een bekend probleem bij neurale netwerken. Het werk dat beschreven wordt in deze thesis is gewijd aan het onderzoek naar continu leren en het oplossen van het fenomeen van vergeten in neurale netwerken.

Bij de aanpak  van het continu leren probleem, gaan we uit van een stapsgewijze methode waar de taken na elkaar volgen en data van de vorige taak niet bewaard blijft.  We starten met de ontwikkeling van een systeem dat tot doel heeft om voor elke taak het expert niveau te benaderen. Het reserveert een apart specialistisch model voor elke taak en leert achtereenvolgens om via een poort de juiste input door te geven aan de corresponderende specialist. Daarna bekijken we het stapgewijs leren van meerdere taken door gebruik te maken van een gedeeld model met een vastgelegde capaciteit. Voor elke taak identificeren we de meest informatieve kenmerken en minimaliseren we de divergentie tijdens het leren van latere taken; met als proxy de data voor de huidige taak.

Als een alternatief voor het zich baseren op de data voor de lopende taak, die misschien een heel andere distributie heeft dan vorige data, kunnen belangrijke parameters in een model geidentificeerd worden, waarbij toekomstige veranderingen een negatieve waarde mee krijgen. Het is echter onmogelijk, als we focussen op een ongelimiteerde sequentie aan taken, om alle informative te bewaren. Als een adaptieve methode voor specifieke testomgeving, stellen we voor om de belangrijkste parameters te leren tijdens het gebruik, terwijl het model actief is in de test omgeving. Het resultaat zal zijn dat het rampzalige ‘alles’ vergeten wordt vermeden, maar elegant selectief vergeten wordt getolereerd. Voor een verdere ontwikkeling van toekomstige taken, bestuderen we de rol van spreiding in continu leren. We stellen een regulator voor die het percentage aan parameters voor elke taak significant beperkt en hierdoor ook het resultaat van het continu leren process aanzienlijk verbetert.

Aangezien de stapsgewijze toename van het leerproces niet in alle gevallen als uitgangspunt genomen kan worden bij continu leren, bestuderen we ook de setting van het on-line continu leren. We gaan uit van een oneindige stroom aan data, afkomstig van een continue distributie met een gecontroleerd of niet-gecontroleerd trainingssignaal. We stellen om te beginnen een protocol voor om ons werk van regularisatie van de belangrijkste parameters over te zetten op  de on-line continu leren setting en daarmee laten we een verbetering in  leren zien voor de verschillende stromen aan data.

Voor het geval van meer uitdagende situaties, waar de distributie van de input een grotere variëteit vertoont, onderzoeken we het gebruik van een vastgelegde buffer van voorbeelden uit de voorgaande reeksen. Wij stellen een voorbeeld van een selectiemethode voor, die  geen veronderstellingen doet over de distributie van gegenereerde data. Voor zover we weten, waren we de eersten om het probleem van on-line continu leren aan te pakken.

De voorgestelde methoden in deze thesis hebben belangrijke aspecten van het continu leren aangepakt. Ze zijn geëvalueerd op verschillende benchmarks en voor verschillende leersequenties. Vooruitgang in de state-of-the-art van het continu leren werd gerealiseerd en de uitdaging om continu leren in de praktijk te kunnen toepassen werd onomstotelijk aangetoond.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
%\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/curriculum/curriculum.tex <==
% !TeX root = ../../thesis.tex
\chapter{Curriculum}\label{ch:curriculum}

Rahaf Aljundi was born on 1988 in Syria. After finishing her secondary school, she studied  computer science engineering at Damascus university, Syria and specialized in artificial intelligence (AI). She graduated among the top ten students and received a prize for her graduation project from ICT
incubator Syria. After graduation, she worked in industry as a software engineer while being a part time teaching assistant and master student in the AI master program, both at Damascus University. In 2012, She was granted a PhD scholarship   from her home university.  However, in 2013, she moved to Europe to start a master program in Machine Learning and Data Mining  which was a joint program between Jean Monnet University, France and University of Alicante, Spain. Her research  during the master's degree was focused on Domain Adaptation for both computer vision and medical imaging.  She was ranked first with honours for the work of her master thesis. 
In October 2015, she joined the Visics group, KU Leuven as a PhD student  under the supervision of prof. Tinne Tuytelaars. In 2016 she received an FWO scholarship for her PhD research which was renewed on 2018.  From Nov 2018 to Feb 2019  she was on a research visit to Montreal institute for learning Algorithms (Mila) working on Continual Learning with dr. Min Lin and prof. Yoshua Bengio.
During her PhD, she worked on continual learning and  published papers in top conferences in Machine Learning and Computer vision including Neurips, ICLR, CVPR, ICCV, and ECCV.  She also served as a reviewer for top machine learning and computer vision conferences and journals.

\instructionscv


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/manual/manual.tex <==
% !TeX root = ../../thesis.tex
\chapter{Manual}\label{ch:manual}


\section{Tips and Tricks}

\subsection{Image on the cover page}

If you want to place an image on the cover of the dissertation, you can add
the code underneath to the template (check with your promotor whether this is
allowed).

\paragraph{Include image:}
Search for the \texttt{\textbackslash frontcoverheaderXII} command in
the \texttt{adsphd.cls} file and add the following lines:
\begin{verbatim}
   \begin{textblock*}{56mm}(10mm+#1,15mm)
   \includegraphics[width=56mm,height=20mm]{image/filename}
   \end{textblock*}
\end{verbatim}
Where 56mm is the width, 20mm the height, 10mm the x-location and 15mm the
y-location.

\paragraph{Change cover font color:}
Add the command \texttt{\textbackslash color\{red\}} to the
\texttt{\textbackslash frontcoverheaderXII} command or enclose specific parts.
For example, \texttt{\{\textbackslash color\{red\}\textbackslash
textbf\{\textbackslash @authorf\textbackslash\ \textbackslash @authorl\}}.

\subsection{Full cover page}

\textbf{Important}: most printing services will create their own cover page based
on the details you send them (title, name, affiliation, ...) and do not supply
you with all necessary parameters (e.g., thickness of the paper) because these
differ from machine to machine. Therefore, the generated cover page is only
indicative and probably not used by your printing server (or even correct).


A full cover page (combining front cover, spine and back cover) can be
generated automatically using the command \texttt{make cover} or \texttt{python3 run.py cover}. This creates a pdf
\texttt{\$(COVERPDF);} by default this is \texttt{cover.pdf}.

The width of the spine is set by redefining \texttt{\\adsphdspinewidth} (9mm by default).

It can be seen in the provided \texttt{thesis.tex} that all information necessary to
generate a cover page is contained between two markers

\begin{verbatim}
    %%% COVER: Settings %%%
    ...
    %%% COVER: End settings %%%
\end{verbatim}

DO NOT REMOVE THESE!! They are used by the Makefile!!

The default front and/or back cover page can be overwritten: 

\begin{itemize}
    \item create a file \texttt{mycoverpage.tex}
    \item redefine the commands \texttt{\textbackslash makefrontcovergeneral} and \texttt{\textbackslash makebackcovergeneral}. For
          an example and more information, see the provided file \texttt{mycoverpage.tex}.
\end{itemize}

The cover page in the generated pdf has the following structure:

{\tiny
\begin{verbatim}
    <--rbleed--><--backcoverpage--><--lbleed--><--spine width--><--lbleed--><--frontcoverpage--><--rbleed-->
\end{verbatim}
}

The default bleed (both lbleed and rbleed) is 7mm. I suggest not changing this
value unless you know what you are doing ;) The latter can be done by
redefining \texttt{\textbackslash defaultlbleed} and \texttt{\textbackslash defaultrbleed} respectively.


\subsection{Table of contents}

To remove list of figures, tables and other preface chapters from the table of
contents, search for occurrences of \texttt{\textbackslash addcontentsline} in the file
\texttt{adsphd.cls} and comment them.

\subsection{Small ebook size}

When you add the \texttt{epub} option to the adsphd class the dissertation is
printed to a smaller size to read on a device such as Kindle.

Environments such as tables or tikZ pictures are often sized in absolute values
and not relative to the size of the output. You can wrap them in a resizebox
to enforce scaling:

\begin{verbatim}
  \resizebox{\textwidth}{!}{%
    \begin{tabular}{cc}
      ...
    \end{tabular}
  }
\end{verbatim}

\section{Settings for TeXstudio}

If you are working with TeXstudio or other windows latex editors you might want to adjust the editor's settings to allow a proper compilation of the table of contents and list of figures/tables.

\subsection{Custom \textit{makeindex} and \textit{makeglossaries} commands}

According to the \textit{README.md} the tables are indexed through two custom commands. To edit them in TeXstudio open the \textit{Commands} settings (\textit{Options $\to$ Configure TeXstudio...,  Commands} sheet), edit the following fields and press OK.

\textit{Makeindex}:
{\scriptsize
\begin{verbatim}
"C:/Program Files/MiKTeX 2.9/miktex/bin/x64/makeindex.exe" %.nlo -s nomencl.ist -o %.nls
\end{verbatim}}

\textit{Makeglossaries}:
{\scriptsize
\begin{verbatim}
"C:/Program Files/MiKTeX 2.9/miktex/bin/x64/makeindex.exe" %.glo -s %.ist -t %.glg -o %.gls
\end{verbatim}}

Now the customized commands can be launched by using \textit{Tools $\to$ Commands $\to$ MakeIndex/Makeglossaries}. If you want to automatize it in the standard \textit{Build \& View} (F5) and \textit{Compile} (F6) commands look at the following section.

\subsection{Custom Build\&View and Compile meta-commands}

Open \textit{Options $\to$ Configure TeXstudio...,  Build} sheet, edit the following field and press OK.

\textit{Build \& View}:
{\footnotesize\begin{verbatim}
	txs:///pdflatex | txs:///bibtex | txs:///makeglossaries | txs:///makeindex |
	txs:///pdflatex  | txs:///pdflatex
	\end{verbatim}}

To view the PDF once created you have to press F7 (or \textit{Tool $\to$ View}) and the PDF will automatically update in the default viewer whan you modify it. 

If you prefer to directly view the created PDF\textbf{ from the beginning }edit the field as follow:
{\footnotesize\begin{verbatim}
	txs:///pdflatex | txs:///bibtex | txs:///makeglossaries | txs:///makeindex |
	txs:///pdflatex  | txs:///pdflatex | txs:///view-pdf
	\end{verbatim}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage



==> chapters/preface/preface.tex <==
% !TeX root = ../../thesis.tex
\chapter*{Acknowledgements}                                  \label{ch:preface}
Obtaining a PhD with impactful research was a target that I set 4 years ago. Working towards this target was not an easy task at all. Without the support of many people, this wouldn't have been possible. 

I would like to express my deepest appreciation to my supervisor prof. Tinne Tuytelaars for her continual support during the course of my PhD. I am especially thankful for the  freedom and the trust that I was given to pursue the research I am passionate about. I wouldn't have been able to proceed without your guidance.  

I am also thankful to prof. Matthew Blaschko for the great mathematical discussions.
I would like to thank my PhD committee prof. Van Gool, prof. Van Hamme,  prof. Vogels,  prof. Vedaldi and prof. Neuckermans for their careful reading of my PhD manuscript, the fruitful discussions, and insights.  

My research was funded by FWO whose vision inspired me to explore continual learning, my beloved topic. I would like to thank them for the trust and I wish my work met their expectations. 

During my PhD I have collaborated with many awesome researchers. Jay Chakravarty,  with him I have got my first two papers. Amal, with her I started  a crazy rush towards a deadline in two months and we won a paper and a friendship. Francisca who joined the lab for a short period but we shared best moments of hard work and laugh. I am really thankful for getting to know you. Klaas, thanks for making our last CVPR paper realizable.

I would like to express my thanks to  Marcus Rohrbach and Mohammed Elhosieny  for the fruitful collaboration and the great discussions on Continual Learning.  During my last research visit to Mila, I had the chance to work with prof. Yoshua Bengio, Min Lin, Eugene Belilovsky, Massimo Caccia and Lucas Caccia. It was the shortest period in which I got to learn the most and survive the freezing Montreal. 


Working towards a PhD can't be done without sharing the best and tough moments with the friends and colleges of Visics and without the help of the friendly staff (Annitta, Bert, Patricia and Paul). Special mention to Bert, Davy and Ali with whom I spent an unforgettable week in Hawaii. Jose, I would like to thank you for the expert answers whenever I needed and for the TITAN X that made my experiments achievable.   


This thesis is dedicated to my parents who planted the seeds of science in me, whose  circumstances didn't support their research path. I hope I have achieved your dream.  My parents, brothers, and sister, without your support I wouldn't have the chance to pursue my career. 

Finally, my biggest lovely thanks go to my husband, Mostafa, who stood by me in each moment of this endless deadlines journey,  listened to my complaints, my worries and never stopped putting confidence in me.  
%\instructionspreface


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/publications/publications.tex <==
\chapter{List of Publications}



\paragraph{Book chapters}
\begin{itemize}
\item Unsupervised Domain Adaptation based on Subspace Alignment. B Fernando, R Aljundi, R Emonet, A Habrard, M Sebban and T Tuytelaars, Domain Adaptation in Computer Vision Applications; Springer, Cham, 2017. 81-94
\end{itemize}
\paragraph{International peer reviewed conferences}
\begin{itemize}
   \item Gradient based Sample Selection for Online Continual Learning. R Aljundi, M Lin, B Goujaud, and Y Bengio in 2019 Conference on Neural Information Processing Systems (Neurips'19).
    \item Online Continual Learning with Maximally Interfered Retrieval. R Aljundi*, L  Caccia*, E  Belilovsky*, M Caccia*, M  Lin, L  Charlin, T  Tuytelaars in 2019 Conference on Neural Information Processing Systems (Neurips'19).
\item Task-free continual learning. R Aljundi*, K  Kelchtermans*, T Tuytelaars   in   Computer Vision and Pattern Recognition (CVPR'19).
\item Selfless Sequential Learning. R Aljundi, M Rohrbach and T Tuytelaars in International Conference on Learning Representations (ICLR’19).
\item Exploring the Challenges towards Lifelong Fact Learning. M Elhoseiny, F Babiloni, R Aljundi, M Rohrbach and T Tuytelaars  in Asian Conference on Computer Vision (ACCV’18).
\item Memory Aware Synapses: Learning what (not) to forget. R Aljundi, F Babiloni, M Elhoseiny, M Rohrbach and T Tuytelaars  in European Conference on Computer Vision (ECCV’18).
\item Encoder Based Lifelong Learning AR Triki*, R Aljundi*, M Blaschko and T Tuytelaars in International Conference on Computer Vision (ICCV'17). 
\item Expert Gate: Lifelong Learning with a Network of Experts. R Aljundi, P Chakravarty, T Tuytelaars in Computer Vision and Pattern Recognition (CVPR'17).
\item Who’s that Actor? Automatic Labelling of Actors in TV series starting from IMDB Images. R Aljundi*, P Chakravarty*, T Tuytelaars in Asian Conference on Computer Vision (ACCV'16).
\item Landmarks-based Kernelized Subspace Alignment for Unsupervised Domain Adaptation R Aljundi, R Emonet, D Muselet and M Sebban In Computer Vision and Pattern Recognition (CVPR’15).

\end{itemize}
\paragraph{International peer reviewed workshops}
\begin{itemize}
\item Lightweight Unsupervised Domain Adaptation by Convolutional Filter Reconstruction. R Aljundi, T Tuytelaars in   TASK-CV: Transferring and Adapting Source Knowledge in Computer Vision workshop (ECCV'16).
\item Transfer Learning for Prostate Cancer Mapping Based on Multicentric MR imaging databases. R Aljundi, J Lehaire, F Prost-Boucle, O Rouvière and C Lartizien In Machine Learning meets Medical Imaging workshop (ICML’15).

\end{itemize}

\paragraph{Under review}
\begin{itemize}

    \item Continual learning: A Comparative Study on How to Defy Forgetting in Classification Tasks. M  De Lange, R Aljundi, M Masana, S  Parisot, X  Jia, A Leonardis, G Slabaugh, T  Tuytelaars. Submitted as a journal paper to TPAMI.
\end{itemize}


==> mycoverpage.tex <==
% Redefine in this file the commands to generate the front and back cover:
%
%   \makefrontcovergeneral{xskip}{clearpage}
%   \makebackcovergeneral{xskip}{clearpage}
%
% You can start from their definition in adsphd.cls. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% My own cover page
\makeatletter

%% \renewcommand{\makefrontcovergeneral}[2]{%
%%   %
%%   % Create header
%%   \frontcoverheader{#1}
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Title, subtitle, authorname, text and date can be moved around.
%%   % Change the textblock* commands below. 
%%   %
%%   % Syntax of textblock environment:
%%   % 
%%   %   \begin{textblock*}{width}(xpos,ypos)
%%   %     ...
%%   %   \end{textblock*}
%%   % 
%%   % !! Make sure not to remove the '+#1' part!!!
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Place the title
%%   \begin{textblock*}{120mm}(17.5mm+#1,89.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \raggedright\selectfont\LARGE\sffamily\textbf{\@title}
%%   \end{textblock*}
%%   %
%%   % Place the subtitle
%%   \begin{textblock*}{120mm}(17.5mm+#1,92.0mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \Large\sffamily{\@subtitle}
%%   \end{textblock*}
%%   %
%%   % Place the author name
%%   \begin{textblock*}{120mm}(17.5mm+#1,109.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \Large\sffamily\@authorf\ \MakeUppercase\@authorl
%%   \end{textblock*}
%%   %
%%   %\begin{textblock}{120}(0,115)
%%   \begin{textblock*}{120mm}(17.5mm+#1,132.0mm)
%%   \textblockcolour{}
%%   \includegraphics*{image/coverfigure}
%%   \end{textblock*}
%%   %
%%   % Place the misc text
%%   \begin{textblock*}{60mm}(96.5mm+#1,187.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   {\small\sffamily Dissertation presented in partial\\
%%   fulfillment of the requirements for\\
%%   the degree of Doctor\\
%%   in \@degree}
%%   \end{textblock*}
%%   %
%%   % Place date
%%   \begin{textblock*}{160mm}(0mm+#1,221.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \begin{center} {\small\sffamily\@date }\end{center}
%%   \end{textblock*}
%%   
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Add footer
%%   \frontcoverfooter{#2}
%% 
%% }

\makeatother

